Learning the Language of Protein Structure

Representation learning and \emph{de novo} generation of proteins are pivotal computational biology tasks. Whilst natural language processing (NLP) techniques have proven highly effective for protein sequence modelling, structure modelling presents a complex challenge, primarily due to its continuous and three-dimensional nature. Motivated by this discrepancy, we introduce an approach using a vector-quantized autoencoder that effectively tokenizes protein structures into discrete representations. This method transforms the continuous, complex space of protein structures into a manageable, discrete format with a codebook ranging from 4096 to 64000 tokens, achieving high-fidelity reconstructions with backbone root mean square deviations (RMSD) of approximately 1-5 \AA. To demonstrate the efficacy of our learned representations, we show that a simple GPT model trained on our codebooks can generate novel, diverse, and designable protein structures. Our approach not only provides representations of protein structure, but also mitigates the challenges of disparate modal representations and sets a foundation for seamless, multi-modal integration, enhancing the capabilities of computational methods in protein design.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

==> sources/01_introduction.tex <==
\section{Introduction} \label{sec:intro}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% generic intro: what is protein
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% what is protein
Protein are often referred to as the workhorse of the living organism and sustain a wide variety of biological mechanisms acting for instance as messengers or catalyzing chemical reaction. 
Conversely, a protein that fails to perform its natural function can have severe implications, potentially leading to conditions like Alzheimer's disease.
% why structure matters
In that regard, protein structure holds a crucial role.
Indeed, favored by a mechanistic view of physico-chemical processes happening in living organisms, the conformation of a protein dictates its function XXCITEXX.
% where is research 
The works oriented towards a better understanding of the protein folding mechanism cover more than 50 years of research and span various fields from physical modeling \citep{Anfinsen1973, Alford2017} to recent machine learning \citep{Jumper2021}.
% Why we should pursue research on that topic: % drug design & understanding of biological proceses
The final objectives of such works also vary.
One of the great promises of Machine Learning based protein structure prediction is the ability to speed-up or unlock protein design to solve health issues, see \citep{OVCHINNIKOV2021}.
It can also provide crucial insights to understand biological processes. 


% Increase in computes & data enables new methods
% new pdbs entries each year 14k,
Protein structure is also at the heart of a data-centric evolution. 
For instance, the number of experimental resolutions of protein structures drastically increased over the last few years with more than 14 thousands new structures added each year onto the ProteinDataBank \footnote{\url{https://www.rcsb.org/stats/growth/growth-released-structures}}.
Other sources of data such as AlphaFold \citep{Jumper2021} or RoseTTaFold \citep{Baek2021} predictions, completes the landscape of protein structures with an accuracy close to experimental resolution \citep{Terwilliger2024}.
Inline with these remarks, we aim to investigate whether the recent advancements of discrete space autoencoders, which have shown promise in representation learning and generation tasks for modalities like images \citep{Razavi2019} and audio \citep{dhariwal2020,defossez23}, can be effectively applied to protein structures. 
%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% New opportunities
%%%%%%%%%%%%%%%%%%%%%%%%%
% ML Conceptual, Parti, Muse
Leveraging discretization techniques, these approaches have overcome previous limitations, exemplified by pioneering efforts in text-conditioned image generation.
Central to their effectiveness is the adoption of highly expressive latent priors, facilitating robust sampling processes that yield high-quality sample, as developed by frameworks such as Parti \citep{Yu2022} and Muse \citep{Chang23b}. 
Our hypothesis is that by transforming continuous features derived from protein structures into discrete codes, quantized-protein structure autoencoders can effectively capture crucial structural information while simplifying the data's complexity.
This discrete representation offers advantages in efficient storage and manipulation of protein structures, making it well-suited for various downstream tasks such as protein function prediction and structure-based drug design. 
Notably, besides generation, recent advancements in bi-lingual language models now propose to incorporate both structural and amino acid information to achieve state-of-the-art performance on multiple downstream tasks \citep{su2024}.

The main contributions of our work are:
\begin{enumerate*}
    \item The introduction of a state-of-the-art protein structures autoencoder with a discrete latent space.
    \item The learning of a generative prior over the learned discrete latent space.
    \item A thorough validation of the generative model notably via self-consistency metrics.
\end{enumerate*}


==> sources/02_method.tex <==
\section{Method} \label{sec:method}
We now describe our proposition to learn an autoencoder with quantized latent space.
The rest of this section is organized as follow: in \cref{subsec.data}, we introduce the setting we adopt to solve the task and
\cref{subsec.architecture} presents the chosen architecture. 
Finally, we detail our training method and some hyperparameters in \cref{subsec.training}.

\subsection{AutoEncoding Protein Structures} \label{subsec.data}
Our objective is to address the learning of an expressive autoencoder with discrete latent space for protein structures. 

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{images/VQ3D.pdf}
    \caption{Schematic overview of our proposition. A protein structure is first encoded as a graph to extract features from using a GNN. This embedding is then quantizied before being fed to the decoder to estimate positions of all backbone atoms} \label{fig.overview}
\end{figure}


\paragraph{Data Source}
Our protein structure data is sourced from the Protein Data Bank (PDB). 
We chose to model the positions of four heavy backbone atoms in each residue: $\N-\CA-\C-\OO$.
This choice is motivated by the backbone's role as a chain-of-atoms that spans the entire protein via covalent bonds, essentially defining the protein's overall shape.
Recent trends in research \citep{Yim23,Wu2024} also adopts this approach. 


\paragraph{Challenges}
Accurately encoding and generating this backbone is pivotal, yet challenging. From a computational standpoint, it requires predicting all backbone atom positions in the protein. This task is intrinsically difficult due to several factors. Firstly, long-range interactions play a significant role in determining the backbone's conformation. Additionally, maintaining the symmetries inherent in the data, particularly the $\mathtt{SE}(3)$ invariance, presents a challenge. Therefore, our objective is to learn discrete representations of protein backbones that preserve invariance under rigid transformations (rotation and translation).


\paragraph{Learning Setting}
For all $n$ residues of our protein, we aim at modeling the position of the backbone atoms  $\N-\CA-\C-\OO$. 
For a protein of length $n$, the data to model is therefore a position vector $p\in \RR^{n\times4\times 3}$ (a position vector for each atom in the backbone for all residues in the protein).
Our main goal is the learning three parametric components: {-- an} encoder ${e_\theta}$ extracting an embedding $z$ from a structure $p$, {-- a} quantization method ${q_\phi}$  discretizing the previously estimated representation, {-- a} decoder $d_\psi$ sending the quantized representation back into the space of protein structures. 
The learnable parameters are respectively denoted $(\theta, \phi, \psi)$ and the learning setting summarizes as:
\begin{equation*}
    p \overset{e_\theta}{\longmapsto} z \overset{q_\phi}{\longmapsto} z_q \overset{d_\psi}{\longmapsto} \hat{p}
\end{equation*}


\paragraph{Backbone Representation for Encoding}
Atoms within a molecule are held together by chemical bonds, which can take various forms such as covalent or ionic bonds. %, inherently creating a graph structure. 
%Several methods exists to represent this graph among which SMILES strings (compact molecular notation at the atom level using text) see \citep{Atz2021})
This structure can be represented as a graph $\mathcal{G}= (\mathcal{V}, \mathcal{E})$, where $\mathcal{V}$ is the set of nodes (that can be atoms for small molecules or residues for proteins), and $\mathcal{E}$ is the set of edges representing the bonds between nodes.
When incorporating positional information into data representations, the following graph-based description naturally emerges: each node (atom) and edge (bond) are associated features that may include positional information (relative distance, angle information etc...) \cite{Fang2022}. 
These graph-based methods, leveraging geometric information, have proven effective in tackling essential protein-related tasks such as inverse folding \citep{Dauparas2022} and predicting protein function or interfaces \citep{Gligorijević2021, Krapp2023}. 
%These results prove the quality of the representation learned by GNN on protein graphs.
We therefore chose to second these works adopting a similar approach to encode structural information.

\paragraph{Backbone Representation for Decoding}
As discussed, protein structures lend themselves naturally to a graph representation with geometric attributes. 
While one approach suggests mirroring the encoding for decoding, retrieving the full structure from a graph may be difficult or impractical.
An alternative approach, exemplified by \citep{Eguchi2022}, uses pairwise distance matrices. 
However, protein structures naturally manifest as point clouds, alleviating the need to solve an inverse problem or expensive post-processing to obtain the actual structure \citep{anand2019fully, Lee2022}.
Therefore, we propose to combine a graph viewpoint for encoding and a point cloud representation for decoding, parameterizing protein atoms with Cartesian coordinates or angles.
This approach for decoding aligns with established practices in protein structure generation, as demonstrated by works such as \citep{bose2024,Yim23}.
% seeing a protein as a graph as inputs:
% why: literature and quite natural: close "interacts more": first molecules and protine and why it has been useful
% seeing protein backbon as a pointcloud for output:
% why matrix distance reprensentation (solving an inverse pb to decode)

A schematic overview of our proposed workflow is depicted in \cref{fig.overview}.

\subsection{Architectures Details} \label{subsec.architecture}

Our autoencoder comprise three main parts that are learned jointly: 
1. A Message Passing Neural Network, encoding geometrical information. 
2. A Quantizer, providing a discretized representation of the embedding of the GNN.
3. A Decoder, that maps the discrete representation back into the structure space.


\paragraph{GNN-Encoder}
Drawing inspiration from the successes reported in \citep{Dauparas2022}, we have chosen to parameterize our encoder using a Message-Passing Neural Network (MPNN). This approach aligns with recent advancements that demonstrated its efficiency in capturing the intricate relationships within molecular graphs.
More precisely, in our setting the graph $\mathcal{G}= (\mathcal{V}, \mathcal{E})$ is as follows: $\mathcal{V}$ is the set of residues and $\mathcal{E}$  indicates a link between connected residues.
We utilized as edge features kernelized distances between $\CA$ atoms (i.e. a Gaussian kernel with various scaling parameter) and use positional encoding as initial node features alongside orientation information. 
The graph sparsity is set to $50$ neighbours per residue.
Further information is available in \cref{app.data_proc}.
The encoding process can be summarized as first graph construction and featurization, with $p$ the inital protein with $n$ residues,  
\begin{equation}
    p \in \RR^{n \times 4 \times 3}  \mapsto (\mathcal{G}, \mathcal{E}) \in \RR^{n \times p_1} \times  \RR^{n \times n \times p_2} \label{eq.feature_gnn} ,
\end{equation}
where $p_1, p_2$ refer respectively to the node and edge embedding dimension. The GNN $e_\theta$ uses nodes and edges features to produce a representation $z$ of dimension $p_3$:
\begin{equation}
  e_\theta: (\mathcal{G}, \mathcal{E}) \mapsto z \in \RR^{n \times p_3}   \label{eq.gnn}.
\end{equation}


\paragraph{Down-sampled Representation} As of now, our learning scheme produces one code (or token) $z_q$ per residue. 
This might be impractical for light-weight applications. 
To address this limitation, we introduce a cross-attention mechanism enabling to effectively reduce the number of codes down by a factor $f$.
This is implemented as stacking 3-layers of down-sampling layers as illustrated in \cref{alg.downsampling}, the initial queries being defined as positional encodings.
Note that this scheme enables to make queries conditional to the input as soon as the second layer.

\begin{algorithm}
\caption{Down/Up-sampling Layer \label{alg.downsampling}}
\begin{algorithmic}[1]
\STATE \textbf{Input:} $\texttt{Queries}, \texttt{Inputs}, \texttt{Mask}$
\STATE \textbf{Output:} $\texttt{Queries}, \texttt{Inputs}$ 
\STATE $\texttt{Queries}=\texttt{CrossAttention}(\texttt{Inputs}, \texttt{Queries}, \texttt{Mask})$ \label{eq.downsampling}
\STATE $\texttt{Queries} =\texttt{MLP}(\texttt{Queries})$  and  $\texttt{Inputs} =\texttt{MLP}(\texttt{Inputs})$ \label{eq.downsampling}
\STATE \textbf{return} $(\texttt{Queries}, \texttt{Inputs})$
\end{algorithmic}
\end{algorithm}

We also preserve the locality of information, we use a local attention masking in the down-sampling layer so that each down-sampled node aggregates information from a small number of neighboring nodes in the sequence space. 
We detail this mechanism in \cref{app.archi}.
Finally, a similar cross-attention process is used for decoding and producing coordinates at the residue level, only varying the size of the initial input queries.



\paragraph{Quantizer}
The pioneering VQ-VAE work \citep{Oord2017} marked a significant step in discrete representation learning, laying the groundwork for a growing field of research.
Following this, subsequent studies have expanded on this foundation: \citet{Razavi2019} improved codebook structures with hierarchical learning, \citet{Zeghidour2021} enhanced codebook usage and expressivity with residual vector quantization, and \citet{Esser2020} used adversarial frameworks to refine codebook learning for better generation. 
However, while previous work has focused on explicit codebook learning, we take a different approach by adopting scalar quantization, using an implicit codebook following principles from \citet{balle2017}. 
Specifically, we follow the refined framework of bounded scalar quantization as described in \citep{Mentzer2024}. 
Let $z$ be some latent representation in $\RR^p$.
\cite{Mentzer2024} propose to learn a bounded low dimensional encoding of $z$ denoted $z_q \in \mathbb{R}^d$, with typically $d\leq8$. 
More precisely, $z_q$ writes as:
\begin{equation}
    z_q = \frac{L}{2} \text{tanh}(W.z) \label{eq.fsq},
\end{equation}
Where $W\in \mathbb{R}^{d\times n}$, and $L$ is a positive integer that controls the span of $z_q$. 
The variable $z_q$ is then rounded up to the nearest integer and the optimization is conducted using a straight-through gradient estimator.
As defined by \cref{eq.fsq}, $z_q$ can only take a finite number of values, hence defining implicitly a codebook.
Finally, the size of the codebook is determined by both $L$ and $d$: small values for $d$ and $L$ result in codebooks with a small number of codes.

\paragraph{Decoding Quantization}
Regarding the decoding architecture, we align with recent research \citep{Yim23} building upon \citep{Jumper2021} and use AlphaFold-2 structure module as decoder.
AlphaFold-2 structure module predicts the position of each atom in the residue.
To do so, AlphaFold impose a parameterization of the point cloud using \textit{frames}.
A frame is defined by a two-uple $(R, t)$: $R$ is the frames' orientation (i.e. a rotation matrix) and a $t$ is the frame center (i.e. vector defining the translation of the center of the frame).
The center is the $\CA$ carbon, and the orientation is defined using the nitrogen and
the other carbon atom.
The structure module prediction is two fold.
A first component involving the IPA modules updates the frame i.e. orientation and position of the $\CA$ atom (for each residue).
A second learnable component, a ResNet, predicts the remaining atoms positions.
For a thorough and mathematical description, we defer to \citep{Jumper2021}.



\subsection{Training Details} \label{subsec.training}


\paragraph{Loss Function}
The Frame Align Point Error (FAPE), introduced in AlphaFold-2 is a function enabling the comparison between point clouds.
Indeed, it is not guaranteed that the coordinates provided by the decoding module are expressed in the same basis as the initially encoded data, thereby crippling the possibility to compare directly the coordinates of both points clouds.
This is the core idea of the FAPE loss: to express coordinates in a comparable frame to compute the mean squared error.
To do so, given a frame $T_i$, and its prediction $T^p_i$, and let $x_j$ be some true atom position and $x^p_j$ be the predicted ones,
the FAPE Loss writes then as:
\begin{equation}
\mathcal{L}_{FAPE}=\|{T_i^p}^{-1}(x^p_j) - T_i^{-1}(x_j) \|\label{eq.fape}
\end{equation}
In \cref{eq.fape}, we compare the coordinates of atom $j$ expressed in the frame of the residue $i$.
This enables the joint optimization of both the predicted frames and coordinates.
In this work, we use the clamped version of the FAPE Loss since we found that it provides more stable training.


\paragraph{GNN Hyperparameter}
We use a 3 layer message passing neural networks as encoder following the architecture and implementation  proposed in \citep{Dauparas2022}. 
We utilize \texttt{swish} activation function.
% edges features: only Ca (as we do) or all-to-all (as protein MPNN)

\paragraph{Decoder Hyperparameter}
We strictly follow AlphaFold implementation regarding the implementation of the structure module using 6 structure layers.
AlphaFold structure module expects a two fold representation as input: $(s_i)_{i \leq N}$ that accounts for the representation of a single residue and $(z_{i,j})_{i,j \leq N}$ that represents pairwise information between residues $i$ and $j$.
We utilise as $s_i$ the re-projected quantized codes.
We describe in \cref{algo:pairwise_representation}, \cref{app.archi} the construction of the pairwise representation $(z_{i,j})_{i,j \leq N}$ used for reconstruction.



%\begin{figure}
%    \centering
%\includegraphics[width=0.5\textwidth]{images/generated_structures.png}
%\caption{Protein Generated using VQ3D=2252 and GPT=272 and using temperature sampling}
%    \label{fig.placeholder figure}
%\end{figure}

\section{Methods}

\subsection{Protein Structure Autoencoder}

Our objective is to train an autoencoder that maps protein structures to and from a discrete latent space of sequential codes.  Following prior works  \citep{Yim23,Wu2024} we consider the backbone atoms of a protein, $\N-\CA-\C-\OO$, to define the overall structure.  For a protein with $N$ amino acids, the structure is therefore given by a tensor of per-atom coordinates of shape $\mathbf{p}\in \RR^{N\times4\times 3}$.  Given a desired downsampling  ratio of the tokenizer, $r$, the latent representation is of a form $\mathbf{\tilde{z}} = [ \tilde{z}_0, \dots, \tilde{z}_{N/r} ]$ where  $0 \leq z_i \in \mathbb{Z} \leq {K-1}$ with $K$ the size of the codebook.

A schematic overview of the our autoencoder is depicted in \cref{fig.overview}.   In this section, we focus on the three parametric components of our model; the \emph{encoder} (${e_\theta}$) extracting a set of embeddings for each residue $\mathbf{z} \in \RR^{N/r}$ from the structure $p$, the \emph{quantization} method (${q_\phi}$) that discretizes the representation to obtain $\mathbf{\tilde{z}}$, and the \emph{decoder} that reconstructs a structure from the quantized representation $\mathbf{\hat{p}}\in \RR^{N\times4\times 3}$.
The learnable parameters are respectively denoted $(\theta, \phi, \psi)$ and the learning setting summarizes as:
\begin{equation*}
    \mathbf{p} \overset{e_\theta}{\longmapsto} \mathbf{z} \overset{q_\phi}{\longmapsto} \mathbf{\tilde{z}} \overset{d_\psi}{\longmapsto} \mathbf{\hat{p}}.
\end{equation*}

\paragraph{Encoder}

Pargraph 1: intuition/description.
\begin{itemize}
    \item Encoder maps protein structures ($\mathbf{\hat{p}}\in \RR^{N\times4\times 3}$) to a continues, and possibly downsampled, tensor of continuous variables $\mathbf{z} \in \RR^{N/r}$.
    \item We observe that this task is reminiscent of mapping protein structure to sequences (i.e.\ inverse folding); a well study task for which many models exists.
    \item Building on this, we choose to model our encoder architecture on ProteinMPNN; where a graph neural network extracts per-residue embeddings from a structure, that are then projected to the desired output.
    \item In our case, as we are interested in a latent representation rather than protein sequence, we can either take these embeddings directly, or use a simple cross-attention layer to obtain the desired output.
\end{itemize}

(Pargraph 2: specific implementation)
Concretely, we,
\begin{itemize}
    \item Provide summary of GNN encoder with reference to ProteinMPNN and/or appendix for full details.
\end{itemize}

\paragraph{Quantization}

Pargraph 1: intuition/description.
\begin{itemize}
    \item What does the quantizer need to do.
    \item Note that while it is most common for methods to directly learn the codebook (e.g.\  \citep{Oord2017, Razavi2019, etc}, we found these methods were less stable during training and prone to codebook collapse (...explain what this is...).
    \item  Therefore, instead we leverage the recenrlt proposed framework of bounded scalar qunatization (FSQ).
\end{itemize}

(Pargraph 2: specific implementation - I copy what we have here but notation and wording can be refined...)
Let $z$ be some latent representation in $\RR^p$.
\cite{Mentzer2024} propose to learn a bounded low dimensional encoding of $z$ denoted $z_q \in \mathbb{R}^d$, with typically $d\leq8$. 
More precisely, $z_q$ writes as:
\begin{equation}
    z_q = \frac{L}{2} \text{tanh}(W.z) \label{eq.fsq},
\end{equation}
Where $W\in \mathbb{R}^{d\times n}$, and $L$ is a positive integer that controls the span of $z_q$. 
The variable $z_q$ is then rounded up to the nearest integer and the optimization is conducted using a straight-through gradient estimator.
As defined by \cref{eq.fsq}, $zw_q$ can only take a finite number of values, hence defining implicitly a codebook.
Finally, the size of the codebook is determined by both $L$ and $d$: small values for $d$ and $L$ result in codebooks with a small number of codes.

\paragraph{Decoder}
\emph{Paragraph 1: intuition/description.}
\begin{itemize}
    \item What does the decoder need to do.
    \item Once again noting the similarity of our task to protein folding (sequence to structure) we repupose the structure module of AlphaFold...
\end{itemize}

\emph{Paragraph 2: specific implementation}

\subsection{Training}

\paragraph{Objective}

\paragraph{Data}
\begin{itemize}
    \item Currently in 4.1.
\end{itemize}

\paragraph{Hyperparameters}
\begin{itemize}
    \item Model hyperparams.
    \item Training hyperparams. (currently in 4.2)
\end{itemize}

==> sources/03_experiment.tex <==
\section{Experiments} \label{section:experiments}
The primary focus of our work is do develop and effective method to encode and quantize 3D structures with high fidelity.  In this section we first evaluate, both qualitatively and quantitatively, our vector-quantized autoencoder by considering the compression and reconstruction performance.  Once we have demonstrated that our tokenizer indeed permits high-accuracy reconstruction of protein sequences, we further highlight how this can be adapted to downstream tasks, by training suprisingly effective \emph{de novo} generator of unseen protein structures using a vanilla GPT model.

\subsection{Autoencoder Evaluation}

\paragraph{Experiments}
We trained six versions our vector-quantized autoencoder; using small ($K=4096$ codes) and large ($K=64000$) codebooks, and increasing the downsampling ratio ($r$) from 1 to 4.  For each codebook we then evaluated the reconstruction performance achieved on the held out test set, to understand the trade-off's between compression and expressivity associated with these hyperparameter choices.

\paragraph{Metrics}
To assess the reconstruction performances of the models, we rely on standard metrics commonly used in structural biology to asses the similarity of two protein structures.
The \emph{root mean square distance (RMSD)} between the input and reconstructed protein backbones is computed by calculating the square root of the average of the squared distances between corresponding atoms of the two structures after optimal superposition. The \emph{TM-score} is a normalised measure of how similar two structures are, with a score of 1 denoting the structures are identical.
To aide in interpreting our results, a pair of structures are commonly said to be experimentally indistinguishable if their RMSD is below 2\AA and are deemed to have similar fold when their TM-score exceeds 0.5 \citep{Xu2010}.

\paragraph{Results}
Our results are summarised in \cref{tab:experiment_results}.  We find that with a codebook of $K=64000$ and a downsampling of $r=1$; our average reconstruction has $1.59$ \AA RSMD and a TM-score of 0.94.  Whilst further increasing the model capacity may allow these scores to be improved even further, this is already approaching the limit of experimental resolution (which is to say, the reconstruction errors are on par with the experimental errors in resolving the structures) which we consider to be a reasonable upper limit of the accuracy we could want.

\input{sources/ablation_table}

We can also see that indeed increasing the downsampling factor or decreasing the codebook size correspondingly impacts reconstruction accuracy.  This is expected as we essentially enforce greater compression in our autoencoder leading to a loss of information - neverthless in all cases we find that the achievable reconstruction performance is still within a few angstrom with TM-scores exeeding our 0.5 threshold on average.
That increasing codebook size also increases performance is also evidence that our method is less prone to codebook collapse (i.e.\ only a subset of the codes being used by the trained model), an issue we faced with several prior quantization methods before adopting FSQ.
 
The reconstruction performance is illustrated in \cref{reconstruction}, where examples of the model's outputs are superimposed with their corresponding targets. 
Visually, our model demonstrates its ability to capture the global structure of each protein. 
Additionally, our model faithfully reconstructs local conformation of each protein preserving essential secondary structures elements of the protein such as the $\alpha$-helices and $\beta$-sheets.

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{images/reconstruction.png}
\caption{
    Visualisation of the model reconstruction super-imposed with the original structures. Each row shows a different structures seen from a different rotation angle (column). The length and reconstruction RMSD are also given on the left of the most left column.
}
\label{reconstruction}
\end{figure}

\subsection{\emph{De novo} protein structure generation} \label{exp.generation}

\paragraph{Experiment}
Given a tokenizer of protein structures, we now turn our attention to demonstrating that this can be effectively leveraged for downstream tasks.  In particular, we consider generation of protein structures from a model trained in our latent space as a paradigmatic demonstration of our tokenizers utility. This is not just because generative models for \emph{de novo} protein design are of great interest for drug discovery -- enabling rapid \emph{in silco} exploration of the design space -- but also as it directly leverages our compressed representation of protein structures using established sequence modelling architectures.

Specifically, we tokenize our dataset (defined in \cref{subsection:Training details}; full details on dataset preparation for this experiment can be found in \Cref{app.gpt_training_details}) using a downsampling factor of 1 and a codebook with 4096 codes (first line of Table~\ref{experiment_results}).
We then train an out-of-the-box GPT model with 344M parameters on the training split.
The obtained generative model is then be used to predict XXX new sequences of tokens which are then converted to 3D protein structures using our pre-trained decoder.

\paragraph{Metrics}
We evaluate the generated structures on different aspects: \emph{designability} (also called \emph{self-consistency}), \emph{novelty} and \emph{diversity}.
\emph{Designability} uses ProteinMPNN \cite{REF!} to predict a sequence given the generated structure and then refolds this using ESMFold \cite{REF!} to report the structural similarity between the original and redesigned structure.  The intuition is that generated structures should be sufficiently natural that established methodologies recognise them and agree on the fundamental biophysical properties.  Moreover, a useful generative model will provide structures that are varied and not simple replications of the training data.  
To asses this, we measure  the \emph{diversity} and \emph{novelty} of our generation.
Diversity refers to the number of modes sampled when generating and is defined using structural clustering, more specifically we report the number of clusters divided by the number of generated sequences.
Novelty is estimated by comparing the generated structure with a dataset of reference and reporting the TM-score with the closest match.
Overall, we follow \citep{Yim23} for the implementation of these metrics and refer the reader to \Cref{app.metrics} for more details on the validation pipeline.


\paragraph{Baselines}
To contextualise our results, we also provide those of FrameDiff \citep{Yim23} and RFDiffusion \citep{Watson2023}; two methods for \emph{de novo} generation of protein structures.
Both of these models leverage bespoke SE(3) diffusion models specifically designed and published for this task.

We emphasise that there are considerable differences between the design objectives of all three models.  RFDiffusion leverages extensive pre-training on a large dataset and requires considerable computational cost for state-of-the-art performance. FrameDiff leverages a SE(3)-invariant diffusion process based on a geometrical decomposition whilst being considerably more lightweight. On the contrary, our generation model is a simple vanilla GPT and the objective here is to show how one can immediately and easily use the tokenized representation learned with our method for protein design.

\paragraph{Results}
Results are summarised in Table~\ref{tabres}.
It is noteworthy that while not specifically designed for the protein structure generation task, even a simple GPT model is able to generate protein structures that are competitive in term of designability to methods specific to protein design such as FrameDiff. As for novelty, it is important to note that while structures that are novel and different from the reference dataset, structures that differ too much from the natural proteins found in the reference dataset, can also indicate unrealistic structures. It is also worth mentioning that the baselines have been trained on XX with higher overlap with the chosen reference dataset than our training dataset. Diversity is tbc.
Extended results and additional analysis are provided in Appendix~\ref{app.add_res}.

\input{sources/results}

% Again, we want to highlight that RFDiff better both because pretraining on large data and complex and tailored diffusion models but method competitive even with off the shelf generic GTP.

==> sources/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The efficiency of our protein structure tokenizer is demonstrated through qualitative and quantitative analyses. We also illustrate how our method can be applied to downstream tasks, particularly in generating novel, diverse, and structurally viable protein structures.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: The limitations of our method stem from the underlying architectures and methods used. For instance, our encoder's limitations are linked to the Message-Passing Neural Network \citep{Dauparas2022}. Similarly, the limitation of our quantization comes from the Finite Scalar Quantization framework \citep{Mentzer2024} while our decoder architecture and configuration follow the structure module of \cite{Jumper2021}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: We use publicly available dataset for all our experiments. We provide details description of the model architecture and will make the code publicly available (redacted to maintain anonymity at this stage).
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: While we recognize the importance of reporting error bars or other measures of statistical significance to avoid drawing false conclusions, we opted not to include them for two main reasons. Firstly, the computational cost of training multiple models with different seeds for each architecture was prohibitively high. Secondly, since our objective was not to achieve state-of-the-art results or claim superiority over existing methods, we deemed the statistical significance of our results less critical in this context.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification:
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> sources/gpt_hyperparams.tex <==
\begin{center}
\begin{table}
\centering
\begin{tabular}{@{}ll@{}}
\toprule
Name &  \\ \midrule
$n_{layers}$   & 20      \\
$n_{heads}$  & 16     \\
$d_{model}$   & 1024     \\
$k/q -\text{size}$   & 64     \\
\bottomrule
\end{tabular}
\vspace{1em}
\caption{Transformer Decoder-Only model hyper-parameters.}
\label{tab:gpt_params}
\end{table}
\end{center}


==> sources/related_works_old.tex <==
\section{Related Works} \label{sec:related}

\paragraph{Learning from Protein Structures.}
Learning from protein structure is thriving research field that encompasses a wide variety of tasks crucial task. 
For instance, inverse folding \citep{Ingraham19,hsu22a,Dauparas2022,jing2021learning} or binding site estimation \citep{Krapp2023,ganea2022independent} are critically enabling for drug design \citep{Scott2016}. 
Others \citep{GeneOntology, robinson2023contrasting, kucera2023proteinshake, Gligorijević2021} focus on learning from protein structure to provide a better understanding of the role of the structure, hence pushing the knowledge frontier of biological processes. 



\paragraph{Representation Learning of Protein Structures.}
\citep{Eguchi2022} learns a VAE using as inputs matrix distances and predicting 3D coordinates. The supervision is done by comparing distance matrices.
Despite the straightforward nature of sampling from a VAE latent space, it often yields subpar sample quality, see \citep{Kingma2016}.
Foldseek \citep{vanKempen2024} propose to learn a VQ-VAE on small chunks of protein comparing true and reconstructed local geometrical features.
Because of the locality of the data used in Foldseek, decoding only small chunks of structures, this quantization defines an interesting tool for efficient structure database search but does not enable full backbone structure sampling. 
Closer to our work, \cite{gao2023vqpl} propose a quantized autoencoder of protein structures, with however only limited reconstruction performances limiting its applicability. 



\paragraph{Generation of Protein Structures.}
A substantial body of literature addresses the challenge of sampling the protein structure space. 
Numerous studies have advocated for the use of diffusion-based models \cite{Wu2024, Yim23, Watson2023} or flow matching techniques \citep{bose2024}. 
While many of these works, such as those by \citep{Yim23, Watson2023, bose2024}, employ complex architectures to ensure invariance to rigid-body transformations, \citep{Wu2024} opted for an alternative parameterization directly preserving symmetries allowing the authors to capitalize on conventional architectures, yet working only on small protein crops. % (< 128 residues).
